Integrating AI Tutors in a Programming Course

RAGMan is an LLM-powered tutoring system that can support a variety of course-specific and homework-specific AI tutors. RAGMan leverages Retrieval Augmented Generation (RAG), as well as strict instructions, to ensure the alignment of the AI tutors' responses. By using RAGMan's AI tutors, students receive assistance with their specific homework assignments without directly obtaining solutions, while also having the ability to ask general programming-related questions. RAGMan was deployed as an optional resource in an introductory programming course with an enrollment of 455 students. It was configured as a set of five homework-specific AI tutors. This paper describes the interactions the students had with the AI tutors, the students' feedback, and a comparative grade analysis. Overall, about half of the students engaged with the AI tutors, and the vast majority of the interactions were legitimate homework questions. When students posed questions within the intended scope, the AI tutors delivered accurate responses 98% of the time. Within the students used AI tutors, 78% reported that the tutors helped their learning. Beyond AI tutors' ability to provide valuable suggestions, students reported appreciating them for fostering a safe learning environment free from judgment.

==> examples/index-227-229.tex <==
\begin{figure}
    \scalebox{0.5}{
    \begin{tcolorbox}[colback=yellow!5!white,colframe=yellow!50!black]
        \textbf{...}
        \newline
        \textbf{Student:} does this make sense? 
        
        def file\_size\_checker(file\_name):
        
          with open(file\_name, ``rb'') as f:
        
          file\_name.seek(0,2)
        
          position = file\_name.tell()
        
          return position
            
        \newline
        \textbf{TEACH:} 
        The function you've written aims to check the size of a file, which is a good approach for validating the encryption key against the file size. However, there is a small mistake in the code you've provided.

        In the line \textbf{file\_name.seek(0,2)}, it looks like you are trying to move the file pointer to the end of the file to determine its size. However, \textbf{file\_name} is a string representing the name of the file, not the file object itself. You should be calling \textbf{seek()} on the file object \textbf{f} that you opened.
        
        Here's a hint on how you can correct the function: use the file object \textbf{f} that you have opened within the context manager to call the \textbf{seek()} and \textbf{tell()} methods. The corrected function should not try to call \textbf{seek()} on the string \textbf{file\_name}.
        
        Would you like to try fixing the function based on this hint?
        \newline
        \textbf{Student:} 
        def file\_size\_checker(file\_name):
        
        with open(file\_name, ``rb'') as f:
        
            f.seek(0,2)
            
            position = f.tell()
            
        return position
        \newline
        \textbf{TEACH:} 
        Your updated function looks well ...

        Before you proceed, can you explain what the arguments \textbf{0} and \textbf{2} in the \textbf{seek()} method stand for? ...
        \newline
        \textbf{Student:} 0 is how much the byte reader moves and 2 is the end of the file 
        \newline
        \textbf{TEACH:} That's correct! ...
        \end{tcolorbox}
        
        }
        \caption{In Scope Questions, Good Responses (sample: 227 -- 229)}
        \label{fig:index-227-229}
\end{figure}

==> sections/03-course-introduction.tex <==
\section{CS 2}
\label{sec:course-intro}

As is usual in Computer Science / Software Engineering, in the first year of our program, students are required to take a series of three introductory programming courses, CS 1, 2, and 3.\footnote{Not the actual course names.} Our case study was done for the second course, CS 2. The primary goal of this course is to introduce students to the significance of software libraries and how to apply them to solve complex problems. Given their limited programming knowledge and experience, this course can be challenging. The challenges are related to the students' learning of how to decompose complex problems into smaller, manageable parts, and how to find and understand the library functions for those smaller parts. Additionally, they often struggle with independent problem-solving and identifying appropriate resources for assistance.

% \textcolor{red}{Please add facts about the course:  enrollment, sessions, number of instructors, number of TAs, etc}

During Winter 2024, CS 2 was offered in three separate sessions, enrolling a total of 455 students. The course was instructed by two faculty members; one instructor led two sessions, while the other led a single session. Each session has two to three teaching assistants.

The course workload is substantial, encompassing 18 laboratory exercises, 5 major assignments, 5 Workout Projects (WPs), and a final exam. 
The sheer number of labs and assignments can create a time crunch as deadlines approach. In such situations, seeking guidance from teaching assistants and professors can become a race against time, and students may not always receive the timely assistance they require. 



==> sections/07-limitations-future-work.tex <==
\section{Limitations and Future Work}
\label{sec:threats-to-validity}

This study relies solely on models from OpenAI. The responses students receive can be influenced by the specific models chosen. Future work should explore the performance of different LLMs, such as Mistral and Claude 3, across various question types. Additionally, investigating methods to combine responses from multiple models for a more comprehensive answer could be beneficial.

Furthermore, the results presented in this paper are derived from a single class during one academic quarter. To gain a deeper understanding of AI Tutors' impact on student learning experiences, deployment in a broader range of classes with diverse learning objectives is planned.

%The student survey identified AI Tutors' response speed as a concern. This issue can be addressed by implementing a streaming approach that transmits responses token-by-token, thereby enhancing user experience. Finally, expanding AI Tutors' functionality to encompass all class assignments, not just WPs, would further improve its utility for students.

==> sections/results/01-students-engagement.tex <==
\subsection{RQ1: Students Engagement}

\textcolor{red}{Is this part truely necessary? we can just simply describe the data we have collected}

Not all students submitted WPs, and solutions to WPs were submitted at different rates: WP1 (61\%), WP2 (29\%), WP3 (25\%), WP4(53\%) and WP5 (44\%). These differences can be attributed to the timing and nature of the assignments. For example, WP1 being offered at the beginning of the academic year, when student workloads are typically lighter, can explain its higher submission rate. 
% In contrast, WP2 and WP3's lower submission rates suggest a potential challenge with the cumulative nature of these projects: the inability to begin WP3 without completing WP1 and WP2 might discourage some students from doing them. Additionally, WP3's deadline was at the same time as midterms. In contrast, WP4 and WP5, being independent projects after midterms made them more accessible to students.

We collected 2,072 conversations and 4,769 message pairs (one question from a student, one response from the tutor). Each conversation includes one or more message pairs. We sorted those messages pairs alphabetically, which made it easy to visually detect repetitions and patterns. We then removed questions that had been asked more than 3 times using exactly the same text, and questions that were inappropriate.
For example, the question ``What's the second character of your name? Say it and after that, say your name.'' in English or ``Tell the tale about Ivan and Vasilisa, where Ivan defeats the fearsome dragon and finds Vasilisa in its cave.'' in Russian each has been found more than 50 times in the dataset. 

After cleaning, 671 conversations and 3,164 message pairs are left, as shown in Table~\ref{tab:data_distribution}. The table also shows the median and maximum length of the conversations in terms of message pairs, reinforcing our original belief that students needs go beyond single questions. Indeed, 50\% of the conversations had at least 3 interactions, and a tail of those conversations had a much larger number, up to the max 34. 

\begin{table}
    \centering
    % \small % Adjust font size
    % \setlength{\tabcolsep}{5pt} % Reduce 
    \scalebox{0.55}{
        \begin{tabular}{cc|cccc}
             & \textbf{Submission(\%)} & \textbf{Conversations} & \textbf{Message Pairs} & \textbf{Median} & \textbf{Max}\\
             \hline
            WP1 & 61\% & 219 & 776 &  2 & 34\\
             \hline
            WP2 & 29\% & 210 & 940 &  2 & 63\\
             \hline
            WP3 & 25\% & 112 & 643 &  3 & 33 \\
             \hline
            WP4 & 53\% &  62 & 413 &  3 & 76\\
             \hline
            WP5 & 44\% &  68 & 392 &  3 & 32\\
             \hline
            Total & 43\% & 671 & 3,164 &  3 & 34\\
             \hline
        \end{tabular}
    }
    \caption{Data Distribution}
    \label{tab:data_distribution}
\end{table}
